A Nonlocal Graph-PDE and Higher-Order Geometric Integration for Image Labeling

This paper introduces a novel nonlocal partial difference equation (G-PDE) for labeling metric data on graphs. The G-PDE is derived as nonlocal reparametrization of the assignment flow approach that was introduced in \textit{J.~Math.~Imaging \& Vision} 58(2), 2017. Due to this parameterization, solving the G-PDE numerically is shown to be equivalent to computing the Riemannian gradient flow with respect to a nonconvex potential. We devise an entropy-regularized difference-of-convex-functions (DC) decomposition of this potential and show that the basic geometric Euler scheme for integrating the assignment flow is equivalent to solving the G-PDE by an established DC programming scheme. Moreover, the viewpoint of geometric integration reveals a basic way to exploit higher-order information of the vector field that drives the assignment flow, in order to devise a novel accelerated DC programming scheme. A detailed convergence analysis of both numerical schemes is provided and illustrated by numerical experiments.

==> Graphics/Geometric_Acceleration_Illustration.tex <==
\begin{tikzpicture}[
	box/.style={rectangle,draw,fill=blue!10,node distance=1cm,text 
	width=15em,text centered,rounded corners,minimum height=2em,thick},
	arrow/.style={draw,-latex',thick},
	]
	\draw[fill = gray!20,draw = blue,rounded corners,dashed] (11.5,-5.8) 
	rectangle 
	(19.5,-2.5);
	\draw[draw = black,rounded corners,dashed] (-4.5,-5.8) 
	rectangle 
	(4.6,-1);
	\node[rotate=-90,blue] at (19.3,-4.2) {\textbf{acceleration}};
	\node [box,text width=20em] (Initialization) {\textbf{initialization}: $S^0 
	\in 
	\mathcal{W}$, $h  > 0$};
	\node [above=3cm of Initialization] 
	(Help_Node) {};
	\node [box,right=3.7cm  of Help_Node 
	,fill=green!10, text width=20em] 
	(initial) {Labeling $\mc{S}^{\ast}$ as minimum of the nonconvex functional 
	\eqref{eq:S-Flow_Pot} \begin{equation*}
	\min_{\tikzmarknode{simplex}{\highlight{red}{$S \in \mathcal{W}$}}} 
	J(S) = -\frac{1}{2}\langle 
	\tikzmarknode{omega}{\highlight{red}{$\Omega$}} S,S \rangle\end{equation*} 
	\begin{tikzpicture}[overlay,remember 
		picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
		\path (omega.south) ++ (0.3,-1.7cm) node[anchor=south 	
		west,color=red!67] (scalep){\textbf{nonlocal connectivity}};
	 	\draw[color=red!57](omega.south) |- 
	 	([xshift=-0.6ex,color=red]scalep.south east);
	 	\path (simplex.south) ++ (0.3,-2cm) node[anchor=south 
	 	west,color=red!67] 
	 	(mean){\textbf{manifold constraint}};
	 	\draw[color=red!57](simplex.south) |- 
	 	([xshift=-0.3ex,color=red]mean.south 
	 	east);
	\end{tikzpicture}};
	\node [rectangle,inner sep=1em] (enclosure) 
	{};
	\node[draw] at (0.2,3.5) {Section \ref{sec:first-order-geometric-DC}};
	\node[draw] at (15.7,3.5) {Section \ref{sec:higher-order-geometric}};
	\node[draw] at (7.8,1.7) {Section 
	\ref{sec:Prel},\ref{sec:Non_Local_PDE}};
	\node [above=0.8em of enclosure,anchor=south,draw,outer 
	sep=0pt,fill=white] (DC_Geom_Second_Order) 
	{\Large\textbf{geometric DC}};
	\node [right=11cm of DC_Geom_Second_Order,anchor=west,draw,outer 
	sep=0pt,fill=white] (DC_Geom_First_Order) 
	{\Large\textbf{accelerated geometric DC}};
	\node[box,right=8.55 cm of Initialization,fill=blue!10] 
	(Initialization_DC) {\textbf{initialization}: $S^0 \in \mathcal{W}$, 
	$\theta_0>0$};
	\node [box,below=0.5 of Initialization_DC] (Choose_Step_Size) 
	{\textbf{stepsize selection} 
		$\tikzmarknode{Step_size_h}{\highlight{green}{$h_k \geq  0$}}$, 
		Algorithm 
		\ref{Geometric_Two_Stage}
		\begin{tikzpicture}[overlay,remember 
			picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
			\path (Step_size_h.south) ++ (-7.5cm,-0.3cm) node[anchor=south 	
			west,draw,fill = green!20] (scalep){if $h_k = 0$};
			\draw(Step_size_h.south) |- 
			([xshift=-0.6ex,color=green!29]scalep.south east);
		\end{tikzpicture}	
	};
	\node [box,below=0.5 of Choose_Step_Size] (Descent_Dir) 
	{\textbf{descent direction} \\ $d_k = \Pi_{0}\Omega 
		S^k+\tikzmarknode{Sec_Or_Field}{\highlight{red}{$\frac{h_k}{2}\Omega 
				R_{S^k}(\Omega S^k)$}}$
		\begin{tikzpicture}[overlay,remember 
			picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
			\path (Sec_Or_Field.south) ++ (-10.3cm,-0.3cm) node[anchor=south 	
			west,color=red!67] (scalep){\textbf{second order information}};
			\draw[color=red!57](Sec_Or_Field.south) |- 
			([xshift=-26.5ex,color=red]scalep.south east);
		\end{tikzpicture}	
	};
	\node [box,below=0.5 of Descent_Dir] (Line_Search) {\textbf{line search} 
	$\to$ $S^{k+1}$};
	\node [box,below=0.5 of Line_Search] (criterion) {\textbf{convergence 
			criterion} ($S^k$ near the boundary)};
	\node[box,below=1 of Initialization,fill=blue!10, text 
	width=20em] 
	(Geom_DC_Update) {\textbf{explicit Euler update:}\\ $S^{k+1} = 
	\exp_{S^k}(h \Pi_{0} \Omega S^k)$, Algorithm 
	\ref{Geometric_Explicit_Euler}};
	\node[box,below=1 of Geom_DC_Update,fill=blue!10, text 
	width=20em] (Conv) {\textbf{convergence criterion}};
	\draw [arrow,bend right] (initial) to 
	(DC_Geom_Second_Order);
	\draw [arrow] (6.95,-1.94) -- (4.6,-1.94)  {};
	\draw [arrow,bend left] (initial) to (DC_Geom_First_Order);
	\path [arrow] (Initialization_DC) -- (Choose_Step_Size);
	\path [arrow] (Choose_Step_Size) -- (Descent_Dir);
	\path [arrow] (Descent_Dir) -- (Line_Search);
	\path [arrow] (Line_Search) -- (criterion);
	\node [box,left=2 of criterion] (output) {final \textbf{labeling}
		$S^{\ast}$};
	\path
	(Initialization.north west) ++(-1em,1em) coordinate (Initialization fit)
	(criterion.north west) ++(-1em,-2.4em) coordinate (criterion fit);
	%\path (criterion.south east) ++(1em,-1em) coordinate (help_1 fit);
	%\path [arrow] (criterion.south) -- ++(0em,-1em) -- (help_1 fit); 
	\draw [arrow] (criterion fit.west) |- (output) 
	node[pos = 0.7,above]{yes};
	\path [draw,thick] (criterion.west) ++(0em,-1em) -- (criterion fit);
	\draw [arrow] (criterion fit) |- (Choose_Step_Size.west);
	\node[left=0.3cm of Descent_Dir] {no};
	%%%% Figure DC  %%%%
	\path
	(Initialization_DC.north west) ++(-1em,1em) coordinate (Initialization_DC 
	fit)
	(Conv.south west) ++(-1em,-1em) coordinate (Conv fit);
	\node [below=2.1cm  of Conv](help_1) {};
	\node [right=-0.385cm  of help_1](help_12) {};
	\node [below=2.255cm  of Conv](help_1_2) {};
	\draw [arrow] (Initialization) to (Geom_DC_Update);
	\path [arrow] (Geom_DC_Update) -- (Conv);
	\draw (Conv) -- (help_1_2) node[midway,left]{yes};
	\draw[arrow] (help_12) -- (output.west);
	\path [draw,thick] (Conv.south) ++ (0em,-1em) -- (Conv fit);
	\draw [arrow] (Conv fit)  |- (Geom_DC_Update.west);
	\node[right=0.5cm of  Conv fit,below] {no};
	

\end{tikzpicture}

==> TexInput/Comparison_FAS_Geometric.tex <==
% !TEX root =  ../NonLocalSFlow.tex

Returning to \eqref{eq:Non_Local_PDE_T0} we note that the pointwise Taylor approximation
\begin{equation}\label{eq:tayler_series_V}
	V(x, t+h) = V(x, t) + \sum_{l=1}^p \frac{h^l}{l!} \frac{\dd^l V}{\dd t^l}(x, t)
\end{equation}
up to order $p$ defines a smoothing step on 
$\mathcal{F}_{\mathcal{V},\mathcal{T}_0\mathcal{W}}$ which may be used in 
\eqref{eq:general_FAS}. 
In particular, by setting $p = 1$ and using \eqref{eq:T0_parameterization2}, we find
\begin{equation}\label{eq:fas_smoothing_ee}
	F_\mathrm{fo}^{(l)}(V_{k}^{(l)}) := (V_{k}^{(l)}, V_{k}^{(l)} + h \Omega^{(l)}\exp_{S_0^{(l)}}(V_{k}^{(l)}))
\end{equation}
akin to a geometric Euler iteration.
For $p=2$ we find
\begin{align}\label{eq:Second_Order_Scheme}
	F_\mathrm{so}^{(l)}(V_{k}^{(l)}) = (V_k^{(l)}, F_\mathrm{fo}^{(l)}(V_{k}^{(l)}) + \frac{h^2}{2}\Omega^{(l)} R_{\exp_{S_0^{(l)}}(V_{k}^{(l)})} \Omega^{(l)} \exp_{S_0^{(l)}}(V_{k}^{(l)}))
\end{align}
by using \eqref{eq:second_derivative}.
Each of these smoothing steps may be applied on either the fine ($l=0$) or coarse ($l=1$) grid.
We will remark on the choice of $\Omega^{(1)}$ in Section~\ref{sec:Exp_Dis}.
\begin{proposition}\label{prop:approximating_two_stage}
	Let $F_\mathrm{fo}$ be a smoothing step on the fine grid and $F_\mathrm{so}$ be a smoothing on the coarse grid. If $I_0^1$ is chosen as injection and the coarse operator $\Omega^{(1)}$ is compatible with restriction at $S(t) = \exp_{S(t)}(V(t))$ in the sense that $I_0^1\Omega S(t) = \Omega^{(1)} I_0^1S(t)$, then the full approximation scheme \eqref{eq:general_FAS} approximates the two-stage scheme \eqref{eq:two_stage_scheme} through
	\begin{subequations}\label{eq:two_grid_scheme}
	\begin{align}
	    \wt S(t)   &\leftarrow \exp_{S(t)}\big( h\Omega S(t) \big)\label{eq:two_grid_scheme1}\\
	           S(t+h) &\leftarrow \exp_{\wt S(t)}\Big( \frac{h^2}{2}I_1^0\Omega^{(1)} R_{I_0^1S(t)} \Omega^{(1)} I_0^1S(t) \Big).\label{eq:two_grid_scheme2}
	\end{align}
	\end{subequations}
\end{proposition}
\begin{proof}
By inserting the specific choice of smoothing steps into \eqref{eq:general_FAS} for $t_k=t$ and $t_{k+1} = t+h$, we find
\begin{subequations}\label{eq:approximation_two_stage_proof}
\begin{align}
	V_{k+1}^{(q+1)} &= V_{k} + h \Omega\exp_{S_0}(V_{k}) + I_1^0 \Big( 
	I_0^1V_{k} + h \Omega^{(1)}\exp_{I_0^1S_0}(I_0^1V_{k})\\ \nonumber
		& \quad +\frac{h^2}{2}\Omega R_{\exp_{I_0^1S_0}(I_0^1V_{k})} 
		\Omega^{(1)} \exp_{I_0^1S_0}(I_0^1V_{k}) - I_0^1 (V_{k} + h 
		\Omega\exp_{S_0}(V_{k})\Big)\\ \nonumber
		&= V_{k} + h \Omega\exp_{S_0}(V_{k}) + I_1^0 \Big( \frac{h^2}{2}\Omega^{(1)} R_{\exp_{I_0^1S_0}(I_0^1V_{k})} \Omega^{(1)} \exp_{I_0^1S_0}(I_0^1V_{k}) \Big)
\end{align}
\end{subequations}
on the tangent space $T_0\mc{W}$. This corresponds to the scheme \eqref{eq:two_grid_scheme} on $\mc{W}$ due to the lifting map action property \eqref{eq:action_property}.
\qed
\end{proof}

\begin{remark}
Because $\wt S(t)$ is available from \eqref{eq:two_grid_scheme1}, one may replace $\Omega^{(1)} \exp_{I_0^1S_0}(I_0^1V_{k})$ in \eqref{eq:two_grid_scheme2} by $I_0^1\wt S(t) = I_0^1\Omega \exp_{S_0}(V_{k})$ which represents the action of $\Omega$ exactly without the need for additional computation.
\end{remark}

==> TexInput/Energy_Decomposition.tex <==
In the preceding sections we argued how a simplest instance \eqref{eq:Explite_Euler}
of geometric integration emerges as a possible numerical scheme for solving 
partial difference equation on the assignment manifold. In the following we 
extend our approach by introducing a two grid geometric integration scheme for 
solving \eqref{eq:Non_Local_PDE} more efficiently.\\[1em]  
For $k \in \N$ let $\mathcal{V}$ be a given rectangular grid graph of size $N 
\times N$ with $N = 2^{k}$ and let $\Omega 
\in \R^{N\times N}$ be the matrix as in \eqref{Help_Lemma}. As in the context 
of multi 
grid solvers for elliptic PDEs \cite{Hackbusch:1985aa} and convex 
optimization problems \cite{Nash:2000aa} we consider the following hierarchical 
grid decomposition 
\begin{align}\label{eq:Decomp}
\mathcal{V}^c \subset \mathcal{V} \subseteq \mathcal{V}^c  
\dot{\cup}\mathcal{V}^c_I \subseteq \mathcal{V}  \dot{\cup}\mathcal{V}_I  
\end{align}       
where $\mathcal{V}^c$ denotes the rectangular grid of size 
$N_c \times N_c$ with $N_c = 2^{k-1}$ after uniform coarsening of $\mathcal{V}$ 
by factor 
2. Reordering the indices of 
$\Omega$ by coarse nodes first and using subscripts $\Omega_{11}$ and 
$\Omega_{00}$ for $\mathcal{V}^c$ and $\mathcal{V}\setminus \mathcal{V}^c$ 
respectively we consider the following matrix decomposition
\begin{align}\label{eq:Reordering}
\Omega = \begin{pmatrix}
\Omega_{11} & \Omega_{10} \\
\Omega_{01} & \Omega_{01} 
\end{pmatrix}, \quad \Omega_{ij} \in \R_{\geq 0}^{N_c\times 
	N_c}, i,j \in \{0,1\},
\end{align}
with the sub matrices $\Omega_{01},\Omega_{10}$ encoding the couplings 
terms on coarse grid $\mathcal{V}^c$ to the fine nodes $x \in 
\mathcal{V}\setminus \mathcal{V}^c$. In the following we write $S = (S^c,S^f)^T 
\in \R^{N_cl \cdot N_cl}$ and derive an equivalent decomposition of the 
objective functional \eqref{eq:S-Flow_Pot} to properly represent the non local 
operator in \eqref{eq:Non_Local_PDE} on coarser grid.

\begin{lemma}\label{Lem:Two_Grid_Dec}
	Let $\Omega \in \R^{N \times N}$ be as in \eqref{eq:Reordering} and let the 
	submatrix $I-\Omega$ be regular.
	Let $I = \mathcal{V}^c \dot{\cup} \mathcal{V}_I^c$ be 
	the domain decomposition as in 
	\eqref{eq:Decomp}. 
	For restriction and prolongation operators respectively given by  
	\begin{align}\label{eq:Schur_Restriction}
	R = \begin{pmatrix}
	I \quad \Omega_{10}(I - \Omega_{00})^{-1} 
	\end{pmatrix}, \quad P = R^T,
	\end{align}
	and using the relation on $\mathcal{V}^c$
	\begin{align}\label{eq:Stoch_Com}
		S_{11} : = R\Omega P = \Omega_{11} + 
		\Omega_{10}(I-\Omega_{00})^{-1}\Omega_{01}
	\end{align}
	the fine grid potential \eqref{eq:S-Flow_Pot} is equivalently represented 
	by non local operators on $\mathcal{V}^c \dot{\cup} \mathcal{V}^c_I$ by
	\begin{equation}
	\label{En_Dec}
	\begin{aligned}
	J(S^f,S^c) &= J_{(\Omega_{00})}(S^f) +
	J_{S_{11}}(S^c) - \langle \Omega_{01} S^c,  S^f \rangle \\ 
	&+ 	\frac{1}{2}\langle 
	\Omega_{01}S^c, 
	R^{0}(P(S^c) \rangle 
	\end{aligned}
	\end{equation}
with $R^0 = (0 \quad I)$ denoting the injection operator on $\mathcal{V} 
\setminus \mathcal{V}^c$.
\end{lemma} 
\begin{proof}
	Applying the decomposition 
	\begin{align}
		(I-\Omega)&= S
		\underbrace{\begin{pmatrix}
		(I-\Omega_{11})-\Omega_{10}(I-\Omega_{00})^{-1}\Omega_{01} &0 \\
		0 & (I-\Omega_{00})
		\end{pmatrix}}_{=:D}
		S^T, \\ &\text{with} \quad
		S =   \begin{pmatrix}
		I & -\Omega_{10}(I-\Omega_{00})^{-1} \\ 
		0 & I 
		\end{pmatrix}
	\end{align}
	and inserting it for the first term in \eqref{eq:S-Flow_Pot} we get 
	\begin{align}
		\frac{1}{2}\langle S, (I-\Omega) S  \rangle &= \frac{1}{2}\langle 
		S^T(S),D S^T (S) \rangle \\ &= \langle P(S^c), D  P(S^c) \rangle  + 
		\frac{1}{2} \langle S^f, (I-\Omega_{00}) S^f \rangle \\
		&\phantom{=}-\langle (I-\Omega_{00})^{-1}\Omega_{01} 
		S^c,(I-\Omega_{00})S^f 
		\rangle\\
		&= \frac{1}{2} \langle S^c,(I-S_{11}) S^c \rangle + 
		\frac{1}{2}\langle 
		(I-\Omega_{00})^{-1}\Omega_{01}S^c, 
		\Omega_{01}S^c\rangle \\ 
		&\phantom{=}+\frac{1}{2} \langle S^f, (I-\Omega_{00}) S^f 
		\rangle - \langle \Omega_{01} S^c,  S^f \rangle \\
		&= \frac{1}{2} \langle S^c,(I-S_{11}) S^c \rangle +\frac{1}{2} \langle 
		S^f, (I-\Omega_{00}) S^f 
		\rangle. \\ 
		&\phantom{=} + 
		\frac{1}{2}\langle 
		\Omega_{01}S^c, 
		R^{0}(P(S^c) \rangle - \langle \Omega_{01} S^c,  S^f \rangle. 
	\end{align}
	Adding the second term in \eqref{eq:S-Flow_Pot} leads the decomposition 
	\eqref{eq:Decomp}.
\qed
\end{proof}  
The coarser matrix $S_{11}$ is again a row stochastic non negative symmetric 
matrix and serves as a natural coarser approximation to 
\eqref{eq:Non_Local_PDE} after Galerkin coarsening with 
\eqref{eq:Schur_Restriction}. In particular the above Lemma shows that the 
minimization process of fine objective functional \eqref{eq:S-Flow_Pot} 
guarantees a descent by solving the non local PDE on a coarser grid by replacing 
the coarsening operator $R$ with a 
simple restriction $I_0^1 = (I \quad 0)$ if the following condition is 
satisfied 
\begin{align}
	\langle \Omega_{01} S^c, R^{0}(P)(S^c) -2S^f \rangle \leq 0.
\end{align}


Building on Lemma~\ref{Lem:Two_Grid_Dec}, we 
approximate the fine energy by the coarse objective 
\begin{align}
	J^c(S^c) = -\frac{1}{2}\langle S^c, S_{11} S^c \rangle
\end{align}
with row stochastic symmetric non negative weighting matrix as introduced in 
\eqref{eq:Stoch_Com}.

==> TexInput/FAS.tex <==
% !TEX root =  ../NonLocalSFlow.tex
In the preceding section we discussed two geometric numerical schemes for integrating the flow \eqref{eq:S-flow-S}.
In view of Proposition~\ref{Prop:Non_Local_PDE}, a natural alternative for 
accelerating numerical computations is to devise a two-grid (or more generally, 
a multi-grid) representation of the PDE \eqref{eq:Non_Local_PDE_T0} by applying 
the full approximation scheme (FAS) from the multigrid literature 
\cite{Briggs:2000aa,Trottenberg:2000aa}. 

Let $\mc{V}=:\mc{V}^{(0)}$ be the vertices of a grid graph of size $N \times N$ with $N = 
2^{\ell}$ for some $\ell \in \N$.
 Consider the hierarchical grid decomposition 
\begin{align}\label{eq:Decomp}
\mc{V}^{(1)} \subset \mc{V}  
 \subseteq \mc{V}  \dot{\cup}\mc{V}_{\mathcal{I}}^{\alpha}  
\end{align}       
where $\mc{V}^{(1)}$ has size $N^{(1)} \times N^{(1)}$ with 
$N^{(1)} = 2^{\ell-1}$ after uniform coarsening of $\mc{V}$ by the factor 2 
along each coordinate, as illustrated in Figure~\ref{fig:Coarseining}.
\begin{figure}
	\captionsetup{font=footnotesize}
	\centering
	\scalebox{0.9}{
	\begin{tikzpicture}
	\draw[radius = 1pt,black] (4.5,2.8) circle[];
	\filldraw[radius = 1pt,black] (4.5,2.3) circle[];
	\node at (5,2.8) {$\in \mathcal{V}_{\mathcal{I}}^{\alpha}$};
	\node at (4.9,2.3) {$\in \mathcal{V}$};
		\draw(1,0) -- (1,3);
		\draw(1, 0) grid[step=0.5cm] (4, 3);
	\filldraw[radius=1pt]
	\foreach \x in {1.5, ..., 3.5} {
		\foreach \y in {0.5,1, ..., 2.5} {
			(\x, \y) circle[]		
		}
	};
\draw[rounded corners=3pt,fill=gray!70,opacity = 0.2]
(1.5,0.5) -- (3.5,0.5) -- (3.5,2.5)--(1.5,2.5);
	\filldraw[radius=1pt]
	\foreach \x in {1.5,2, ..., 3.5} {
		\foreach \y in {0.5,1, ..., 2.5} {
			(\x, \y) circle[]}}
	;
	\draw[radius=1pt,black]
	\foreach \x in {1,4} {
		\foreach \y in {0,0.5, ..., 3} {
			(\x, \y) circle[]
	}};
	\draw[radius=1pt,black]
	\foreach \y in {0,3} {
		\foreach \x in {1,1.5, ..., 4} {
			(\x, \y) circle[]
	}};		
	\draw[radius = 1pt,black] (10.69,2.8) circle[];
	\filldraw[radius = 1pt,black] (10.69,2.2) circle[];
	\filldraw[radius = 2pt,gray] (10.7,1.7) circle[];
	\filldraw[radius = 1pt,black] (10.7,1.7) circle[];
	\node at (11.3,2.8) {$\in \mathcal{V}^{{\alpha}}_{{\mathcal{I}}_D}$};
	\node at (11.48,2.2) {$\in \mathcal{V} \setminus \mathcal{V}^{1}$};
	\node at (11.2,1.7) {$\in \mathcal{V}^{1}$};
	\draw(7,0) -- (7,3);
			\draw
			(7, 0) grid[step=0.5cm] (10, 3)
			;
			\filldraw[radius=2pt,gray]
			\foreach \x in {7.5, ..., 9.5} {
				\foreach \y in {0.5,1.5, ..., 2.5} {
					(\x, \y) circle[]		
				}
			};
		\draw[rounded corners=3pt,fill=gray!70,opacity = 0.2]
		(7.5,0.5) -- (9.5,0.5) -- (9.5,2.5)--(7.5,2.5);
		\filldraw[radius=1pt]
		\foreach \x in {7.5,8.0, ...,9.5} {
			\foreach \y in {0.5,1.0, ...,2.5} {
				(\x, \y) circle[]}};
		\draw[radius=1pt,black]
			\foreach \x in {7,10} {
				\foreach \y in {0,0.5, ..., 3} {
					(\x, \y) circle[]
			}};
		\draw[radius=1pt,black]
		\foreach \y in {0,3} {
			\foreach \x in {7,7.5, ..., 10} {
				(\x, \y) circle[]
		}};		
	\end{tikzpicture}}
	\caption{\textbf{Left:} Fine grid  
	$\mathcal{V}$ with zero boundary conditions imposed 
	on the whole interaction domain $\mc{V}_{\mathcal{I}}^{\alpha}$. 
	\textbf{Right:} The grids \eqref{eq:Decomp} 
	coarse  
	interaction domain $\mathcal{V}^{1}_{\mathcal{I}}$ and zero Dirichlet 
	conditions imposed on $\mathcal{V}_{\mathcal{I}_D}^{\alpha}$. Nodes in 
	$\mathcal{V} \setminus \mathcal{V}^{1}$ captures the outflow from the 
	coarse grid 
	$\mathcal{V}^{1}$ into the fine grid $\mathcal{V}$ by means of a non-zero 
	divergence in \eqref{eq:Non_local_Gauss}. }
	\label{fig:Coarseining}
\end{figure} 
Now let $\wt V^{(q)} = (V_k, V_{k+1}^{(q)})$ denote a discretization of the space-time volume $\mc{V} \times [t_k, t_{k+1}]$ with index $q \in \N$ corresponding to the intermediate two-grid iteration that determines $V_{k+1}$ from $V_{k}$. Here we assume $V_k$ to either be given by the boundary condition \eqref{S_Flow_T0_boundary2} or to be the current iterate computed on $\mc{V} \times [t_{k-1}, t_{k}]$.
%In both cases, $V_k$ is not changed by the inner iteration $q$.
Let $F^{(0)}$ and $F^{(1)}$ denote smoothing operations on the fine and coarse grid, respectively,  and let $I_0^1,I_1^0$ denote restriction and prolongation operators between functions on $\mc{V}=\mc{V}^{(0)}$ and $\mc{V}^{(1)}$.
The general FAS iteration reads
\begin{equation}\label{eq:general_FAS}
	\wt V^{(q+1)}_{k+1} = F^{(0)}(\wt V^{(q)})_{k} + I_1^0 \Big( F^{(1)}(I_0^1 \wt V_{k+1}^{(q)}) - I_0^1 F^{(0)}(\wt V_{k+1}^{(q)}) \Big)
\end{equation}
where the fine grid iterate $F^{(0)}(\wt V_{k+1}^{(q)})$ is corrected by the error $F^{(1)}(I_0^1 \wt V_{k+1}^{(q)}) - I_0^1 F^{(0)}(\wt V_{k+1}^{(q)})$ determined on the coarse grid.
The smoothing operations are to be constructed such that $\lim_{q\to\infty} \wt{V}_{k+1}^{(q)}\to V(t_{k+1})$, where $V(t)$ denotes the exact integral curve of \eqref{eq:T0_parameterization2}.

==> TexInput/Geometric_Integration.tex <==
% !TEX root =  ../NonLocalSFlow.tex



We discuss numerical integration of $S$-assignment flows by leveraging the 
tangent space parameterization \eqref{eq:T0_parameterization}.  For a 
discussion of relations to the geometry of $\mc{W}$, we refer to 
\cite{Zeilmann:2020aa}. 
By applying the explicit Euler scheme to \eqref{eq:T0_parameterization2}, we find the \emph{geometric Euler} scheme on $\mc{W}$ as
\begin{equation}\label{eq:geometric_euler}
    S(t+h) \approx \exp_{S_0}\big( V(t) + h\dot V(t) \big)
           %= \exp_{\exp_{S_0}(V(t))}\big(h\dot V(t) \big) 
           = \exp_{S(t)}\big( h\Omega S(t) \big).
\end{equation}
where the last equality is due to the lifting map action property
\begin{equation}\label{eq:action_property}
  \exp_{S}(V_1 + V_2) = \exp_{\exp_{S}(V_1)}(V_2).
\end{equation}
We compute the second derivative of all component functions on $T_0\mc{W}$ as 
\begin{equation}\label{eq:second_derivative}
    \ddot V(t) = \Omega \frac{\dd}{\dd t}\exp_{S_0}(V(t))
               = \Omega R_{\exp_{S_0}(V(t))} \dot V(t)
               = \Omega R_{S(t)} \Omega S(t).
\end{equation}
The second-order expansion $V(t+h) = V(t) + h\dot V(t) + \frac{h^2}{2}\ddot V(t) + \mathcal{O}(h^3)$ in $T_0\mc{W}$ thus leads to the geometric integration scheme
\begin{subequations}\label{eq:second_order_scheme}
\begin{align}
    S(t+h) 
           %&\approx \exp_{S_0}\Big( V(t) + h\dot V(t) + \frac{h^2}{2}\ddot V(t) \Big)
           &\approx \exp_{S(t)}\Big( h\dot V(t) + \frac{h^2}{2}\ddot V(t) \Big)\label{eq:second_order_scheme1}\\
           &= \exp_{S(t)}\Big( h\Omega S(t) + \frac{h^2}{2}\Omega R_{S(t)} \Omega S(t) \Big),\label{eq:second_order_scheme2}
\end{align}
\end{subequations}
which may be read as the two-stage algorithm
\begin{subequations}\label{eq:two_stage_scheme}
\begin{align}
    \wt S(t)   &\leftarrow \exp_{S(t)}\big( h\Omega S(t) \big), \qquad
           S(t+h) &\leftarrow \exp_{\wt S(t)}\Big( \frac{h^2}{2}\Omega R_{S(t)} \wt S(t) \Big).
\end{align}
\end{subequations}

==> TexInput/Non_Local_PDE.tex <==
% !TEX root =  ../NonLocalSFlow.tex
Using the nonlocal concepts from Section~\ref{sec:Prel},
we next show how the Riemannian flow 
\eqref{eq:S-flow-S} emerges as a particular nonlocal diffusion process.
\subsection{Nonlocal PDE}
Before stating the nonlocal partial difference 
equation, we generalize the notion of local boundary conditions to volume 
constraints on discrete domains. Given an \textit{undirected} graph 
$\mathcal{G} = (\mathcal{V},\mathcal{E},\Omega)$ and an antisymmetric mapping 
$\alpha$ as in \eqref{eq:Interaction_Dom}. 
Following \cite{Du:2012aaD}, natural domains for imposing nonlocal
\emph{Neumann-} and \emph{Dirichlet} volume constraints are given by the 
disjoint decomposition of $\mathcal{V}_{\mathcal{I}}^{\alpha}$
\eqref{eq:Interaction_Dom} as 
\begin{align}
\mathcal{V}^{\alpha}_{\mathcal{I}} = \mathcal{V}^{\alpha}_{\mathcal{I}_{N}} 
\dot \cup 
\mathcal{V}^{\alpha}_{\mathcal{I}_D}.
\end{align} 

\begin{lemma}\label{Help_Lemma}
	Given $f \in \mathcal{F}_{\mathcal{V}}$ and a symmetric mapping $\Theta \in 
	\mathcal{F}_{\mathcal{V}\times \mathcal{V}}$ as in definition 
	\eqref{eq:Non_Local_Dif} let 
	$\overline{\Omega} \in \mathcal{F}_{\mathcal{V} 
		\dot{\cup} 
		\mathcal{V}^{\alpha}_{\mathcal{I}} \times \mathcal{V} 
		\dot{\cup} 
		\mathcal{V}^{\alpha}_{\mathcal{I}}}$ and $\overline{f} \in 
		\mathcal{F}_{\mathcal{V} 
		\dot{\cup} 
		\mathcal{V}^{\alpha}_{\mathcal{I}}}$ be the mappings defined for each 
		$x,y,z \in 
	\mathcal{V} \dot{\cup} \mathcal{V}^{\alpha}_{\mathcal{I}}$ as
	\begin{equation}\label{eq:Omega_Dec}
	\overline{\Omega}(x,y):= \big(\delta_{\mathcal{V}\times \mathcal{V}}(\alpha 
	\circ 
	\Theta \circ
	\alpha)\big)(x,y),\quad
	\overline{f}(z):= \begin{cases}
	f(z), &\quad z \in \mathcal{V}, \\
	0, &\quad z \in \mathcal{V}_{\mathcal{I}}^{\alpha},
	\end{cases}
	\end{equation}
	where $\delta_{\mathcal{V}\times \mathcal{V}}$ is the indicator function on 
	$\Z^{d}\times \Z^{d}$ of 
	$\mathcal{V}\times \mathcal{V}$. Then, denoting the above matrix by 
	$\Omega$ on $\mathcal{V}\times \mathcal{V}$, the following identity 
	holds,
	\begin{equation}\label{eq:Reform_Av}
	\sum_{y \in \mathcal{V} \dot{\cup} 
		\mathcal{V}^{\alpha}_{\mathcal{I}}}\Omega(x,y)f(y) = 
		\frac{1}{2}\mathcal{D}^{\alpha}(\Theta 
	\mathcal{G}^{\alpha}(f))(x)+f(x).
	\end{equation}
\end{lemma}
\begin{proof}
	Using \eqref{eq:Omega_Mat} and \eqref{eq:Omega_Dec}, for each $x \in 
	\mathcal{V}$, we directly get
	\begin{subequations} 
	\begin{align}
	 	\sum_{y \in \mathcal{V} \dot{\cup} 
	 			\mathcal{V}^{\alpha}_{\mathcal{I}}}& \hskip -0.2cm 
	 			\Omega(x,y)f(y) = -\sum_{y 
	 			\in 
	 		\mathcal{N}(x)}\Theta(x,y)\alpha(x,y)^2\Big(-\big(f(y)-f(x)\big)\Big)+
	 		f(x)\\
			&=-\sum_{y \in 
			\mathcal{N}(x)}\Theta(x,y)\big(\mathcal{D}^{\ast}(f)(x,y)\big)
		\alpha(x,y)+f(x)\\
		&=\sum_{y \in 
			\mathcal{N}(x)}\frac{1}{2}\Big(\Theta(x,y)\big(-2\mathcal{D}^{\ast}(f)(x,y)\alpha(x,y)\big)\Big)+f(x)
	%	&= \frac{1}{2}\mathcal{D}^{\alpha}(\mathcal{G}^{\alpha}(f))(x)+f(x)
	\end{align}
	\end{subequations}
	which according to \eqref{eq:Non_Local_Dif} implies the identity 
	\eqref{eq:Reform_Av}.
\qed
\end{proof}
The following 
proposition reveals how the flow \eqref{eq:S-flow-S} can be reformulated as a 
nonlocal partial difference equation. 
\begin{proposition}{\textbf{(S-Flow as nonlocal PDE)}}\label{Lem:Non_Local_PDE}
	With $\Omega$ as in Lemma~\ref{Help_Lemma} and $\alpha(x,y) \neq 0, x,y \in 
	\mathcal{V} \dot{\cup} 
	\mathcal{V}_{\mathcal{I}}^{\alpha}$, the flow \eqref{eq:S-flow-S} 
	admits the representation
	\begin{subequations}\label{eq:Non_Local_PDE}
	\begin{align}
	&\partial_{t}S(x,t) = R_{S(x,t)}\Big( 
	\frac{1}{2}\mathcal{D}^{\alpha}\big(\Theta 
	\mathcal{G}^{\alpha}(S)\big)+S \Big)(x,t),&\quad &\text{ on }  
	\mathcal{V}\times \R_{+},\label{S_Flow_PDE}\\
	&S(x,t) = 0, &\quad &\text{ on } \mathcal{V}^{\alpha}_{\mathcal{I}_D}\times 
	\R_{+} \label{S_Flow_boundary1},\\
	&\mathcal{N}^{\alpha}(\Theta \mathcal{G}^{\alpha}(S))(x,t) = 0, &\quad 
	&\text{ on } 
	\mathcal{V}^{\alpha}_{\mathcal{I}_N}\times 
	\R_{+} \label{S_Flow_boundary3}\\
	&S(x,0) = \overline{S}(x)(0), &\quad &\text{ on } \mathcal{V} \dot{\cup} 
	\mathcal{V}^{\alpha}_{\mathcal{I}} \times \R_+, \label{S_Flow_boundary2}
	\end{align}
	\end{subequations}
	where $\overline{S}(x)(0)$ denotes the extension of $S \in 
	\mathcal{F}_{\mathcal{V},\mathcal{W}}$ as in Lemma~\ref{Help_Lemma}.
	Additionally, the \emph{tangent space parameterization} \eqref{eq:T0_parameterization2} admits the representation
	\begin{subequations}\label{eq:Non_Local_PDE_T0}
	\begin{align}
	&\partial_{t}V(x,t) = \Big( \frac{1}{2}\mathcal{D}^{\alpha}\big(\Theta 
	\mathcal{G}^{\alpha}(\exp_{S_0}(V))\big)+\exp_{S_0}(V) \Big)(x,t), &  
	&\hskip -0.2cm \text{on }  
	\mathcal{V}\times \R_{+},\label{S_Flow_PDE_T0}\\
	&V(x,t) = 0, & &\hskip -0.35cm \text{ on } 
	\mathcal{V}^{\alpha}_{\mathcal{I}}\times \R_{+} 
	\label{S_Flow_T0_boundary1}\\
	&\mathcal{N}^{\alpha}(\Theta \mathcal{G}^{\alpha}(\exp_{S_0}(V))(x,t) = 0, 
	& & \hskip -0.35cm \text{ on } 
	\mathcal{V}^{\alpha}_{\mathcal{I}_N}\times 
	\R_{+} \\
	&V(x,0) = \overline{V}(x)(0), & & \hskip -0.25cm \text{on } \mathcal{V} 
	\dot{\cup} 
	\mathcal{V}^{\alpha}_{\mathcal{I}} \times \R_+. \label{S_Flow_T0_boundary2}
	\end{align}
	\end{subequations}
\end{proposition}
\begin{proof}
	Both \eqref{eq:Non_Local_PDE} and \eqref{eq:Non_Local_PDE_T0} follow 
	directly by applying Lemma~\ref{Help_Lemma} to \eqref{eq:S-flow-S} and 
	\eqref{eq:T0_parameterization2}, respectively. 
\qed
\end{proof}
\begin{remark}
	Imposing zero Dirichlet and Neumann volume constraints on the whole 
	interaction domain in \eqref{S_Flow_boundary1} and 
\eqref{S_Flow_boundary3}, 
	respectively, implies vanishing nonlocal divergence in 
	\eqref{eq:Non_local_Gauss}. This assumption prevents any 
	information outflow from the domain $\mc{V}$ to its complement, which is a 
	natural assumption for problems in mathematical imaging. We refer to 
	\cite{Elmoataz:2015aa} for a comprehensive study treating discrete Laplace 
	operators on weighted graphs. 
\end{remark}
In Section~\ref{sec:Exp_Dis}, we will consider a particular data-driven instance of $\Omega$.
For alternative approaches proposed in the context of image regularization and inpainting, we 
refer, e.g., to \cite{Elmoataz:2008aa} and \cite{Gilboa:2009aa}. 


==> TexInput/Numerical_Algorithm.tex <==
In this section show how geometric integration acts as a solution scheme for 
the non local partial 
difference equation \eqref{eq:Non_Local_PDE} on regular discrete grid 
$\mathcal{V}$ and yields a sequence of states on $\mathcal{S}$ with 
monotonically decreasing values for the objective functional 
\eqref{eq:S-Flow_Pot}. For this purpose we focus on the use of simple explicit 
geometric 
Euler integration scheme which generates a  sequence of 
iterates $\{S\}_{k = 1}^N$ for \eqref{eq:S-flow-S} by 
\begin{equation}\label{eq:Explite_Euler}
	S_{k+1}(x) = \exp_{S_k(x)}(h_k(\Omega S)(x)). \qquad S_0 = 
	\exp_{\mathbb{1}_c}(-\frac{D}{\rho}), 
\end{equation}    
with a time step parameter $h_k> 0$. The next Lemma shows how  
\eqref{eq:Explite_Euler} approximates a local minimum of \eqref{eq:S-Flow_Pot} 
and serves as a finite difference scheme for the nonlocal PDE 
\eqref{eq:Non_Local_PDE}. 
\begin{lemma}\label{Lem:Numerical_Scheme}
	Let $\Omega(x,y)$ be as in Lemma \eqref{Help_Lemma}. Then 
	the explicit geometric integration scheme \eqref{eq:Explite_Euler} is 
	equivalent to a sequence generated by 
	\begin{align}\label{eq:PDE_Euler_Update}
	S_{k+1} = \exp_{S_{k}}\Big(-h_kS_{t_k}-\frac{1}{2}\mathcal{D}(\Theta 
	\nabla_{\alpha}(h_kS_{t_k}))\Big).
	\end{align}
	For each $t_{k+1} > t_{k}$ it holds
	\begin{equation}\label{eq:Dec_Seq_Euler}
		J(S_{k+1}) \leq J(S_{k}). 
	\end{equation}  
\end{lemma}
\begin{proof}
	The equivalence of \eqref{eq:PDE_Euler_Update} follows directly by 
	performing identical step as in \eqref{Lem:Non_Local_PDE} for $\Omega 
	S(x)$. It remains to show that the sequence ${S_{k}}$ satisfies 
	\eqref{eq:Dec_Seq_Euler}. For each $\alpha > 0$ let $J_{\alpha}$ we 
	consider the following generalization of functional \eqref{eq:S-Flow_Pot} 
	\begin{equation}
	J_{\alpha}(S) = \frac{1}{2}\langle S, L_{G} S \rangle - \alpha ||S||^2.
	\end{equation}
	Adding an entropy term $\langle S , \log S \rangle$
	with $\gamma > 0$ we rewrite the above functional as 
	 \begin{align}
	  J_{\alpha}(S) &= \frac{1}{2}\langle S,L_G S \rangle - \alpha ||S||^2 \\
	 &= \underbrace{\gamma \langle S, \log S \rangle}_{ = f_{conv}(S)} + 
	 \underbrace{\frac{1}{2}\langle S,L_G S \rangle - \alpha ||S||^2 -\gamma 
	 \langle S, \log S \rangle}_{f_{conc}(S)} \label{eq:DC_Programm}.
	 \end{align}
	 This is a sum of convex and concave functions where the concavity of 
	 $f_{conc}$ is observed from its Hessian 
	 \begin{equation}\label{eq:Concav_Proof}
	 \begin{aligned}
	 	\nabla^2 f_{conc}(S) &= L_G - \alpha I_n-\gamma \Diag(\frac{1}{S}) \\
	 	& = Q \big((1-\alpha)-\Lambda(\Omega)-\gamma 
	 	\Diag(\frac{1}{S}) \big) Q^T,
	 \end{aligned}
	 \end{equation}
	 where in the last step we used the spectral decomposition 
	 $Q\Lambda(\Omega)Q^T$ of $\Omega$. For each eigenvalue $\lambda$ of the 
	 first term on the right side of \eqref{eq:Concav_Proof} we have 
	 \begin{equation}
	 |\lambda| 
	 \leq 2-\alpha-\frac{\gamma}{S} \leq 2 - \alpha-\gamma.
	 \end{equation}
	 Therefore setting $\alpha = 1$ and $\gamma  \geq 1$ yields the concavity 
	 of $f_{conc}$. Setting $h(S):= -f_{conc}(S)$ Equation 
	 \eqref{eq:DC_Programm} is now a particular case of 
	 DC programming and using the Fenchel inequality for $h(S)$ we minimize 
	 the following upper bound at current iterate $S_k$
	 \begin{align}
	 	J_{\alpha}(S_k) = f_{conv}(S_k)-h(S_k) \leq 
	 	f_{conv}(S_k)+h^{\ast}(S_k)-\langle S,S_k \rangle,
	 \end{align}
	 with $h(\tilde{S})$ denoting the Fenchel conjugate of $h(S)$. Optimality 
	 condition for minimizing the upper bound and with subgradient inversion 
	 rule we get for $\tilde{S}_{k+1}$
	 \begin{align}\label{eq:First_opt_con}
	 	S_k \in \partial h^{\ast}(\tilde{S}_{k+1}) \Leftrightarrow 
	 	\tilde{S}_{k+1} \in \partial 
	 	h(S_k) = \nabla h (S_k).
	 \end{align}
	Next using convex inequality for $h$ with $\tilde{S}_{k+1}$ and solving for 
	the next iterate yields 
	\begin{align}
		S_{k+1} \in \argmin_{S}(f_{conv}(S))-\langle \tilde{S}_{k+1},S \rangle 
		\Rightarrow 
		\tilde{S}_{k+1} = \nabla f_{conv}(S_{k+1})
	\end{align} 
	Together with \eqref{eq:First_opt_con} this leads to
	\begin{equation}
		\nabla f_{conv}(S_{k+1}) = - \nabla f_{conc}(S_{k}),  
	\end{equation}
	which in our particular case reads
	\begin{align}
		\gamma \log S_{k+1} = L_G S_k- S_k - \gamma \log S_k. 
	\end{align}
	Solving for $S_{k+1}$ with constraint $S_{k+1} \in \Delta_c$ we get 
	\begin{align}
		S_{k+1} = \frac{S_k e^{-\frac{1}{\gamma}\Omega 
		S_k}}{\langle S_k, e^{-\frac{1}{\gamma}\Omega S_k}\rangle},
	\end{align}
	which is \eqref{eq:Explite_Euler} for $1 \leq \gamma = \frac{1}{h}$.
\end{proof}
In particular regarding the task of solving the non local partial difference 
equation stated in Proposition \eqref{Lem:Non_Local_PDE}, Lemma 
\eqref{Lem:Numerical_Scheme} provides an attractive way of using geometric 
integration schemes which minimize the objective \eqref{eq:S-Flow_Pot} for 
small enough step sizes $h \leq 1$. 

==> TexInput/Two_Stage_Convergence_Rates_7_0.1.tex <==
\begin{tikzpicture}
	\begin{axis}[
		%nodes near coords,
		every other node near coord/.append style={font=\tiny},
		legend columns=1,
		legend style={row sep=0.1cm},
		height=8cm,
		width = 10cm,
		legend entries={{\small Alg. \ref{Geometric_Explicit_Euler}},{\small 
				Alg. \ref{Geometric_Two_Stage}}},
		legend pos=north east,
		mark repeat=4,
		xlabel = Number of iterations,
		xmin=100,
		xmax=2000,
		scaled ticks=true,
		/pgf/number format/.cd,
		use comma,
		1000 sep={}
		]
		\addplot[line join=round,mark = square*,color = Layer_4]
		coordinates {(10,146.9823532333927)
			(60,142.71957992460406)
			(110,37.68194847217378)
			(160,31.03927200880349)
			(210,28.351871102236196)
			(260,26.567233400449137)
			(310,25.218698936808348)
			(360,23.734705269133883)
			(410,22.814033559292167)
			(460,22.0450641023518)
			(510,21.473710560364882)
			(560,20.766457149432167)
			(610,19.91840900105779)
			(660,19.147099950500294)
			(710,18.505049955888897)
			(760,17.666685309113504)
			(810,16.890083311191383)
			(860,16.260588133068058)
			(910,15.622374919508013)
			(960,15.129334494732133)
			(1010,14.592251051990505)
			(1060,14.057296063310439)
			(1110,13.396403523446546)
			(1160,12.78966763799944)
			(1210,12.235061556276575)
			(1260,11.652455332003273)
			(1310,11.254684224585578)
			(1360,10.954450258402153)
			(1410,10.535473368481979)
			(1460,10.206571792356575)
			(1510,9.892102337428623)
			(1560,9.510543868124348)
			(1610,8.868066222540207)
			(1660,8.542867314659807)
			(1710,8.1128386954116)
			(1760,7.310520368650601)
			(1810,6.680563000193685)
			(1860,5.578399811764393)
			(1910,4.958740342809342)
			(1960,4.481261873199308)
			(2010,3.923732666349533)
			(2060,2.588240897549121)
			(2110,1.3008631257249095)
		};	
		\addplot[line join=round,mark = triangle*,color = Layer_10]
		coordinates {(10,67.43358821150136)
			(60,35.41567907482965)
			(110,32.0477184961667)
			(160,29.751616644338746)
			(210,25.148708074698263)
			(260,23.50213183893251)
			(310,21.52196688161956)
			(360,20.057508823541482)
			(410,18.770795991777696)
			(460,17.48886252043029)
			(510,16.321810427933958)
			(560,15.382421182011337)
			(610,14.10685140971967)
			(660,12.966225902868883)
			(710,12.315327626596428)
			(760,10.732432684170517)
			(810,9.933398558371005)
			(860,8.540202502427134)
			(910,7.064743866796539)
			(960,6.673586583313453)
			(1010,4.8323373476546365)
			(1060,3.131809657350952)
			(1110,0.49276968800390125)
		};	
		]
	\end{axis}
\end{tikzpicture}
